Runway Sign Classifier: A DAL C Certifiable Machine Learning System

In recent years, the remarkable progress of Machine Learning (ML) technologies within the domain of Artificial Intelligence (AI) systems has presented unprecedented opportunities for the aviation industry, paving the way for further advancements in automation, including the potential for single pilot or fully autonomous operation of large commercial airplanes. However, ML technology faces major incompatibilities with existing airborne certification standards, such as ML model traceability and explainability issues or the inadequacy of traditional coverage metrics. Certification of ML-based airborne systems using current standards is problematic due to these challenges. This paper presents a case study of an airborne system utilizing a Deep Neural Network (DNN) for airport sign detection and classification. Building upon our previous work, which demonstrates compliance with Design Assurance Level (DAL) D, we upgrade the system to meet the more stringent requirements of Design Assurance Level C. To achieve DAL C, we employ an established architectural mitigation technique involving two redundant and dissimilar Deep Neural Networks. The application of novel ML-specific data management techniques further enhances this approach. This work is intended to illustrate how the certification challenges of ML-based systems can be addressed for medium criticality airborne applications.

==> 1_introduction.tex <==
Machine Learning (ML) is evolving quickly and has already found its way into safety critical transport applications such as autonomous automobiles \cite{autonomous_vehicles_survery}. The European Union Aviation Safety Agency (EASA) is envisioning a first certification of an airborne ML-based system in 2025, and a full certification of an autonomous commercial aircraft by 2035 \cite{easaroadmap2020}.
However, the huge potential of ML in airborne applications is currently limited by conservative and stringent safety and design assurance practices. Existing standards
for airborne systems have major incompatibilities with certain aspects of machine learning, making
certification problematic \cite{eurocae2021SoC}. Since 2019, the joint EUROCAE/SAE WG-114/G-34 working group is actively developing the new AS6983 standard for airborne ML certification. However, acceptance of a new standard may take a few more years due to the novelty and complexity of the topic and the involvement of many stakeholders (WG-114/G-34 comprised of more than 500 members).

To address these issues, we proposed and implemented a custom workflow to achieve DAL D for a machine learning system using the existing assurance standards DO-178C, ARP-4754A, and DO-254 in our previous works \cite{ML_DALD_Dmitriev_21, ML_case_study_Dmitriev_22}. In this paper, we extend the analysis of our custom workflow to the systems of higher criticality that should comply with DAL C. We study the applicability and sufficiency of the architectural mitigation methods described in ARP4754A and leverage independently developed ML components to achieve the targeted design assurance level. We also analyze several alternative means for ML assurance addressing the ML-specific traceability and coverage issues, and apply in conjunction with architectural mitigation method to enhance the overall assurance confidence for DAL compliance.

In contrast to the known related work \cite{codann_1_2020,codann_2_2020,easaL1concept2021} proposing an essentially new workflow for ML-based applications, our approach is based on the incremental and selective adaptation of the existing assurance practices from low to high criticality. Since we build on top of the principles proven through many years of aviation industry experience, we believe that the proposed approach can be applied for certification of ML-enabled airborne systems right now, without waiting for new standards to be released.

The rest of this paper is structured as follows: in Section~\ref{sec:relwork}, we discuss related work. Section~\ref{sec:arch_mitigation} includes the analysis of architectural mitigation method with respect to design assurance level reduction for ML-enabled systems. Then, we review several alternative mitigation measures for ML-specific problematic assurance objective in Section~\ref{sec:alt_means}. Section~\ref{sec:compliance} includes the detailed analysis of the applicable assurance objectives and overall compliance of the custom workflow with DAL C. Section~\ref{sec:concl} summarizes the work and concludes with suggestions for future work.


==> 2_relatedWork.tex <==
There are several foundational reports prepared by aviation authorities addressing certification aspects of ML-based systems. The European Aviation Safety Agency has published the Artificial Intelligence Roadmap \cite{easaroadmap2020} and the ML application guidance \cite{easaL1concept2021} that provide a detailed set of objectives and means of compliance for certification of ML-based safety critical systems. These reports are not positioned to constitute a final certification guidance but intended to anticipate future airworthiness regulations for ML-enabled systems. EASA together with Daedalean AG have also released the CoDANN I \cite{codann_1_2020} and CoDANN II \cite{codann_2_2020} technical reports describing concepts of design assurance for Neural Networks. These reports provide a detailed study of several ML-specific development and assurance aspects such as explainability and generalization topics and also propose a W-shaped ML development process.

The U.S. Federal Aviation Administration (FAA) also in cooperation with Daedalean AG has published a report on the research project studying the neural network vision-based landing guidance system \cite{FAA_ML_Study}. This report presents in-depth practical evaluation of the W-shaped process proposed earlier in \cite{codann_1_2020} and \cite{codann_2_2020}.

SAE International issued a study that presents a new ML development lifecycle to be considered as a basis for the new EUROCAE and SAE standard AS6983 for AI and ML certification \cite{wg114_ml_cert}. It also provides a survey and comparison of several other recent ML certification studies: \cite{easaL1concept2021,deel_ML,AMLAS_hawkins_2021}.

In comparison to the above listed works, in this paper we specifically focus on DAL C and study the assurance objectives corresponding to this level and affected by ML-related issues. This approach is intended to leverage the most of certification credits from traditional assurance methods, supplemented by the selected mitigation measures for the known ML-specific gaps.

In addition, there are multiple research projects that study various ML-specific verification and validation techniques including structural coverage \cite{DeepXplore,deepgauge,sun2019nnCoverage,cheng2018quantitativeCov} and traceability topics \cite{aravantinos2019traceability,borg_traceability} which we consider as alternative mitigation measures.


==> 3_Arch_Mitigation.tex <==
\begin{figure*}[!hb]
	\centering
	\includegraphics[width=1\columnwidth]{figures/sys_arch.png}
	\caption{System Architecture Variants with Two and Three Dissimilar Components}
	\label{fig:sys_arch}
\end{figure*}

 In this study, we propose to leverage the architectural mitigation means described in ARP4754A \cite{SAE.4754} to approach certification of the DAL C. ARP4754A allows to reduce the design assurance level if a system is implemented by two or more dissimilar components. Therefore, DAL C systems can be designed using two or more dissimilar DAL D components provided that a sufficient level of independence between the components is ensured in order to minimize the possibility of common errors between components and cascade failures (Option~2 in Table~3 ``Development Assurance Level Assignment to Members of a Functional Failure Set'' of ARP4754A). It is also necessary to establish robust partitioning between dissimilar components to avoid potential adverse impact of errors in one component to the other.
 
 Figure~\ref{fig:sys_arch} shows potential modifications of the Runway Sign Classifier system with on a Deep Neural Network (DNN) described in \cite{ML_case_study_Dmitriev_22}. These modifications implement simple redundant architectures of a  DAL C system with two or three dissimilar and partitioned DNN components of different types. Such architectures allow for the reduction of design assurance level for the dissimilar components to DAL D - a level down from the DAL C allocated to the system. The Variant I of the architecture with two dissimilar components can provide sufficient integrity and may be acceptable for systems with lower function availability requirements. The Variant II of the architecture with three dissimilar components is intended to increase the availability of the system function at the cost of higher complexity. Availability and integrity requirements must be determined performing a system safety analysis, e.g. according to ARP4761 \cite{SAE.4761}.
 
 In practice, the redundant architectures may include more dissimilar components as well as sophisticated arbitration and voting features. ASTM3269-21 discusses best practices for run-time assurance architectures that can be applied for architectural mitigation in airborne systems \cite{ASTM.F3269}. An example if practical implementation of a redundant architecture with two dissimilar DNNs and their statistical analysis is presented in \cite{SYSAI_He_2022}.

ARP4754A provides only a brief note about system characteristics that can affect independence: ``components with identical hardware and/or software could be susceptible to generic (common cause) faults, which could cause failures in multiple systems'' \cite[p.~107]{SAE.4754}. DO-178C expresses concerns about evaluation of diversity: ``the degree of dissimilarity ... is not usually measurable'' \cite[p.~16]{RTCA.178}.  For demonstration of ML-based components independence, we propose to apply all traditional best practices described DO-178C and ARP4754A, supplemented with ML-specific techniques:
\begin{itemize}
    \item Dissimilar electronic hardware should be used in the independent components, in particular complex hardware elements, such as microcontrollers or FPGA that cannot be exhaustively tested as, defined in EASA CM-SWCEH-001 \cite{EASA.CM-HW-001}.
    \item Software of the independent components should be developed by different persons and cannot include shared code such as compiler libraries. DO-178C guidance for dissimilar software development that include application of different programming languages, compilers, linkers and verification environment should be followed. If off-the-shelve software such as operating systems is used, same principles should be applied.
    \item Requirements and design of the independent components should be developed by different persons to minimize the likelihood of common errors.
%    \item Diverse tools for development and verification of different components should be used, in particular ML-specific tools such as ML training and testing frameworks.
    \item Diverse tools for development and verification of different 
components should be used. 
In particular, ML-specific tools and algorithms used for development and 
design of the ML architecture, handling and analysis of data sets, training of the ML component, as well as verification and testing tools and frameworks need to be considered.
    \item Independent datasets for different ML-based components should be used (ML-specific).
    \item Finally, the common mode analysis of the system as per APR4761 \cite{SAE.4761} should be conducted to evaluate whether the necessary level of independence is achieved or further corrective actions are needed.
\end{itemize}


==> 4_Alt_Verification_Means.tex <==
The architectural mitigation technique discussed in the previous section is a powerful method for the justification of DAL reduction in order to avoid the problematic verification objectives. However, this architectural mitigation method alone may not be fully accepted by certification authorities for the reduction of ML-based system DAL due to the conceptual novelty of ML technology. The EASA guidance does not recommend the reduction of assurance levels through the architectural mitigation, however it is noted that ``... this limitation will be revisited when experience with AI/ML techniques has been gained'' \cite[p.~77]{easaL1concept2021}.

In \cite{ML_DALD_Dmitriev_21}, we identified the DO-178C objectives that cannot be satisfied for ML-based systems due to the fundamental differences between ML-based data-driven technology and traditional software development. In this section we further analyze the unreachable objectives (verification gaps) applicable to DAL C systems and propose alternative methods to mitigate the issues that can be caused by verification gaps identified in \cite{ML_DALD_Dmitriev_21}. These alternative methods can be applied in conjunction with the architectural mitigation technique to strengthen the development assurance confidence and claim DAL C compliance.

In the following analysis we assume, that the custom ML development workflow proposed in \cite{ML_DALD_Dmitriev_21} is followed, and in particular that the ML model represents the low-level software requirements in terms of DO-178C and DO-331.

\subsection{Traceability Issue}
The first major verification gap is the traceability issue: ``.. the DO-178C traceability objectives are not achievable for a ML model'' \cite{ML_DALD_Dmitriev_21}. This verification gap does not impact DAL D systems if the custom workflow proposed in \cite{ML_DALD_Dmitriev_21} is applied. In that workflow, a ML model represents low-level software requirements that can be omitted for DAL D and therefore traceability between ML model and upstream requirements is not required. However, DAL C and higher levels are impacted by this traceability issue because low-level requirements and their traceability are mandatory. 

As ML model behaviour is specified by a set of parameters (e.g., NN weights) adjusted during the training process, in which every parameter is potentially affected by every element of training data, the traditional definition of traceability, in which elements of low-level requirements (represented by ML model) can be isolated and traced to upstream requirements is no longer relevant for ML models. Instead, we can consider and directly address the underlying goals of traceability objectives as explained in DO-248B \cite{RTCA.248B}. With respect to low-level requirements, the traceability has two goals:
\begin{enumerate}
    \item Ensure completeness of the implementation, i.e., all high-level requirements are addressed in low-level requirements.
    \item Support detection of unintended functionality, i.e., all requirements identified as non-traceable may represent unintended behaviour and have to be additionally verified as derived requirements. 
\end{enumerate}
We propose qualification of the ML training framework as a mitigation means for this issue. The first goal for implementation completeness can be justified by a qualified ML training algorithm that can ensure that all training data representing upstream ML model requirements are correctly processed and transferred to ML parameters. However, the training algorithm qualification does not guarantee the absence of unintended functionality (second goal). For example, unintended functionality can be present in ML models even before the intended training begins via transfer learning \cite{transfer_learning_Lu}. In addition, it can be noted that elements of pre-trained ML models such as layers, connections and underlying algorithms should be considered as derived (not traceable to upstream level) requirements. Analysis of such requirements with respect to potential adverse impact to system safety, as required by DO-178C, may be hindered by the explainability challenge \cite{deel_ML}.

In summary, the proposed mitigation measure only partially addresses the traceability issue and should be elaborated in the future work. 

\subsection{Requirements Coverage Issue} 
The goal of requirements coverage is to ensure that all functionality specified in requirements is sufficiently verified by testing. As we discussed in \cite{ML_DALD_Dmitriev_21}, a typical ML model such as a DNN of any practical size is not directly explainable by a human with respect to its functional behaviour (explainability challenge \cite{deel_ML}). Hence it is not generally feasible to trace system function tests to individual elements of an ML model and demonstrate complete test coverage of functional requirements expressed by the ML model.
On the other hand, the low-level behaviour of individual ML model elements such as NN layers and their underlying functions can be specified as derived requirements and tested independently from the system functional behaviour. Even though it is not practically possible to trace such ML model elements to the system function that they implement, it is still feasible to specify derived requirements for individual ML model elements and test them based on these requirements. Though this approach does not fully address the issue because the completeness of coverage cannot be confirmed by traceability analysis (\text{traceability issue}), it still increases verification confidence and may be accepted for DAL C when applied concurrently with architectural mitigation. Structural coverage analysis of the ML model discussed hereafter can also contribute to the fulfilment of this objective.

\subsection{Structural Coverage Issue}
The second aspect of the coverage issue considered in \cite{ML_DALD_Dmitriev_21} is the structural coverage problem: \textit{``... even though the DO-178C structural coverage objectives are achievable, they are generally not representative for the ML source code.''} \cite{ML_DALD_Dmitriev_21} because \textit{``... a single randomly picked test input was able to achieve 100\% code coverage''} \cite{DeepXplore}. Several studies suggest different metrics for  structural coverage analysis at ML model level, such as: neuron coverage \cite{DeepXplore}, neuron boundary coverage \cite{deepgauge}, sign-sign coverage \cite{sign_sign_cov}, NLC (NeuraL Coverage) metric \cite{nlc_coverage} and others \cite{DNN-coverage-2020}. There is currently no consensus in the aerospace certification community about the general effectiveness of the suggested metrics \cite{eurocae2021SoC}, so the relevance of metrics should be evaluated on a case-by-case basis for each application. Nonetheless, the analysis of ML model structure coverage with selected metric can contribute to the overall confidence of verification.

On the other hand, we can also consider the underlying goal of the structural coverage analysis to approach this issue. As per DO-178C, the structural coverage analysis is intended to:
\begin{enumerate}
    \item Detect deficiencies in test cases or procedures
    \item Reveal omissions in requirements
    \item Find extraneous source code (unintended functionality)
\end{enumerate}
The first and second goals can be supported by strengthened reviews and analysis of requirements, test cases and procedures. We propose to apply independence, which is not required for DAL C by default, but can be used in ML-based workflows as an additional measure contributing to overall verification confidence. The third goal is problematic, for now there is no agreed solution for detection of unintended functionality in ML models \cite{unintended_func_cofer}. The neural network  coverage metrics discussed above is  a promising approach but needs further study and evaluation.

\subsection{Explainability Issue}
As discussed above, ML model functional behaviour is generally not directly explainable by humans and therefore not verifiable by reviews or inspection. ML model testing with test data sets can be claimed to satisfy most of the verification objectives (compliance, accuracy, consistency and verifiability) \cite{ML_DALD_Dmitriev_21}, similar to the model-based simulation approach described in DO-331 \cite{RTCA.331}. Learning assurance techniques specified in \cite{easaL1concept2021} (verification of ML model performance, stability, robustness, and generalization capabilities) can be used to increase testing confidence. Coverage and traceability objectives discussed above can also be claimed as mitigated by these additional assurance techniques. As future work, we will evaluate techniques for ``out-of-distribution'' detection via ML model boundary coverage as an additional measure to tackle the explainability challenge.

\subsection{Tool Qualification Issue} 
Qualification of ML development tools require additional considerations in addition to the traditionally used RTCA DO-330 standard \cite{RTCA.330}. Due to the generally stochastic concept of the learning problem, a fully qualified training algorithm does not guarantee the correctness of the trained model and therefore, tool qualification provides only limited confidence credit. New tool qualification criteria and levels may need to be introduced to address these issues. We plan to explore tool qualification issue further in future work.


==> BACKUPS.tex <==
\begin{figure*}[!hb]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/Manager_snapshot.png}
	\caption{SimPol Manager Application}
	\label{fig:manager}
\end{figure*}




==> notes.tex <==
Restructure: analysis -> proper assumptions

Spelling (EASA, AI - make capital) in the references

\Konstantin{Describe the outline of the table}

6&\Konstantin{ADD 331 OBJECTIVES}
&x&x&x&x&&\\
\hline

\Konstantin{discuss other gaps listed in \cite{eurocae2021SoC}}

\Johann{That is certainly true, but the preprocessing/post-processing of ML (think NN) might very well be parameterized - but that is traditional SW. Do we need to mention that? (not necessarily).}

\Johann{NN architectures are usually parameterized (e.g., number layers, number nodes, but these parameters are design parameters and this not under this objective. right?}

\TODO{put tables in Appendix or inline in the section content (preferable)}

